Exploring Federated Unlearning: Review, Comparison, and Insights

The increasing demand for privacy-preserving machine learning has spurred interest in federated unlearning, which enables the selective removal of data from models trained in federated systems. However, developing federated unlearning methods presents challenges, particularly in balancing three often conflicting objectives: privacy, accuracy, and efficiency. This paper provides a comprehensive analysis of existing federated unlearning approaches, examining their algorithmic efficiency, impact on model accuracy, and effectiveness in preserving privacy. We discuss key trade-offs among these dimensions and highlight their implications for practical applications across various domains. Additionally, we propose the OpenFederatedUnlearning framework, a unified benchmark for evaluating federated unlearning methods, incorporating classic baselines and diverse performance metrics. Our findings aim to guide practitioners in navigating the complex interplay of these objectives, offering insights to achieve effective and efficient federated unlearning. Finally, we outline directions for future research to further advance the state of federated unlearning techniques.

==> chapters/10-chap-authors.tex <==

\title{A Survey of Federated Unlearning: A Taxonomy, Challenges and Future Directions}


\author{
Yang Zhao$^{5}$\thanks{These authors contributed equally to this work.}
\and
Jiaxi Yang$^{1,4}$\footnotemark[1] 
\and 
Yiling Tao$^1$
\and
Lixu Wang$^3$
\and
Xiaoxiao Li$^4$ \thanks{Corresponding Author}
\and
Dusit Niyato$^5$
\affiliations
$^1$ University of Electronic Science and Technology of China, China, \\
% $^2$Agency for Science, Technology and Research (A$*$STAR), Singapore, \\
$^2$South China University of Technology, China, 
$^3$Northwestern University, USA, \\
$^4$University of British Columbia, Canada,
$^5$Nanyang Technological University, Singapore 
% \emails
% abbottyang@std.uestc.edu.cn,
% s180049@e.ntu.edu.sg,
}

==> chapters/12-chap-tradeoffs.tex <==
 \section{Trade-offs in Federated Unlearning Methods}


\begin{itemize}
\item \textbf{Erasure-Privacy Trade-off.} The trade-off between data erasure and privacy preservation in federated unlearning involves ensuring compliance with privacy regulations, such as GDPR's right to data erasure while safeguarding the privacy of the data during the unlearning process. For instance, the FedRecovery algorithm utilizes differential privacy by adding tailored Gaussian noises to model updates, minimizing the difference between the original and unlearned model after specific data erasure~\cite{zhang2023fedrecovery}. Similarly, the Exact-Fun algorithm leverages the gradient descent with added noise to selectively remove data from the model, which is designed to obscure the trace of the deleted data, ensuring that the model’s output remains consistent before and after the unlearning process~\cite{xiong2023exact}.

\item  \textbf{Privacy-Efficiency Trade-off.} The trade-off balances privacy preservation with unlearning efficiency. Achieving high privacy often increases computational demands, affecting system scalability and speed. Thus, federated unlearning methods ensure the removal of requested data without degrading accuracy. For example, FedLU~\cite{zhu2023heterogeneous} and FedRecovery~\cite{zhang2023fedrecovery} emphasize balancing data privacy with efficient processing and global convergence, without compromising privacy through knowledge distillation and differential privacy strategies. 

\item \textbf{Privacy-Accuracy Trade-off.} The privacy preservation and model accuracy trade-off involves balancing the need for data privacy against maintaining the effectiveness of federated learning models. This balance is crucial as strategies to enhance privacy, such as anonymizing data or employing encryption techniques, might limit the model's access to detailed information, potentially reducing its accuracy. For example, BFU leverages Bayesian methods to update models without sharing raw data, enhancing privacy but facing challenges in retaining model accuracy due to less precise data~\cite{wang2023bfu}. Then, the FedME$^2$ framework employs the Memory Evaluation (MErase) module to selectively erase data, focusing on removing the most privacy-sensitive or outdated information while minimizing the impact on model accuracy.

\item \textbf{Efficiency-Accuracy Trade-off.} This trade-off involves balancing high model accuracy against minimizing the computational overhead to ensure the unlearning process is efficient. Optimizing for efficiency may reduce resource consumption and speed up processes but can potentially impact model accuracy. Effective federated unlearning methods must find a balance that allows for fast unlearning without significantly compromising the accuracy of the federated learning models. For example, the FFMU algorithm utilizes the Nemytskii operator for simultaneous training and unlearning efficiently across models~\cite{che2023fast}. In addition, KNOT localizes unlearning and retraining processes to specific clusters to minimize the computational and communication overheads~\cite{su2023asynchronous}.

\item \textbf{Efficiency-Security Trade-off.}  Efficiency-security trade-off is to balance the efficiency of the federated unlearning method and the security of the federated learning system, especially in scenarios involving data removal from malicious terminals. This balance ensures that the unlearning does not significantly degrade the accuracy of the federated learning model, while still effectively mitigating the risks posed by malicious actors. The framework leverages parameter updates subtraction and additional training with a benchmark dataset to ensure the unlearning process is effective and efficient, maintaining model accuracy while reducing the overall unlearning cost~\cite{guo2023fast}.

\end{itemize}

Therefore, federated unlearning involves balancing multiple trade-offs, including erasure-privacy, privacy-efficiency, privacy-accuracy, efficiency-accuracy, and efficiency-security. These trade-offs highlight the challenges in optimizing both the unlearning process and model integrity while preserving privacy. Existing studies categorize these trade-offs and propose various algorithms to address them, such as FedRecovery, Exact-Fun, FedLU, BFU, FedME$^2$, FFMU, and KNOT. Each method aims to find the optimal balance between privacy, accuracy, efficiency, and security in the federated unlearning process.

==> chapters/2-chap-preliminary.tex <==
\section{Definition of Federated Unlearning}
\label{sec:background}



Specifically, FU allows clients to request for data sample removal, denoted as $\mathcal{S}_{k}$ for client $\mathcal{C}_k$, from the training process, thereby unavoidably affecting the global model $\mathcal{M}$. FU aims to adjust the global model $\theta$ into $\theta^{u}$ to resemble the performance of a model $\theta^{*}$ that is virtually trained from scratch using the residual dataset $\mathcal{D}_k \backslash \mathcal{S}_k$. This objective can be theoretically defined as making the distribution of $\mathcal{M}_{\theta^{*}} (\mathcal{D}_k \backslash \mathcal{S}_k)$ as close to that of $\mathcal{M}_{\theta^{u}} (\mathcal{D}_k)$ as possible. The definition is
\begin{align}
        \mathrm{Pr}(\mathcal{M}_{\theta^{*}} ( \mathcal{D}_k \backslash \mathcal{S}_k ) ) \backsimeq \mathrm{Pr}(\mathcal{M}_{\theta^{u}} (\mathcal{D}_k) ).
\end{align}

Note that here $\mathcal{S}$ varies in terms of different concepts, forming a taxonomy that includes class-level, sample-level, and client-level unlearning as illustrated in Figure~\ref{fig:framework}. In this taxonomy, class-level unlearning aims to remove specific classes from the model's knowledge. Sample-level unlearning focuses on excluding particular data subsets, whereas client-level unlearning involves erasing all data associated with a particular client. Additionally, based on this taxonomy,  we systematically classify the existing literature in Table~\ref{literatures}. 

\begin{figure*}
	\centering{\includegraphics[scale=0.5]{figures/FU.png}}
	\caption{Framework of Federated Unlearning from three different levels: \textit{class-level, sample-level and client-level}.}
	\label{fig:framework}
\end{figure*}

==> chapters/4-chap-efficiency.tex <==
\section{Advanced Federated Unlearning}
\label{sec:efficiency}

Advanced federated unlearning approaches are oriented towards efficient data removal rather than retraining. These approaches use privacy-preserving models, trade-offs between data removal and model accuracy, and tackle issues including data poisoning and membership inference attacks focusing on efficiency, privacy, accuracy, scalability, adaptability, and robustness.


\subsection{Maintain Model Accuracy} 
Federated unlearning attempts to achieve an equilibrium where data is removed from models and model accuracy is preserved. In FedME$^2$, a Memory Evaluation (MErase) module is used to establish which portion of the data within the model is relevant enabling accurate decisions of what to unlearn and minimize the accuracy loss~\cite{xia2023fedme}. Furthermore, its memory guidance fine-tunes the model's weights to mitigate accuracy loss following data erasure, achieving incremental updates that gradually diminish unlearned data's impact. Specifically, FedME$^2$ keeps the impact on the accuracy of global models under $4\%$ at the average data forgetting rate of approximately $75\%$ in the system of federated learning. Similarly, the Bayesian Federated Unlearning (BFU) algorithm facilitates unlearning in federated learning models by leveraging Bayesian methods to update the global model based on the remaining and erased data, without sharing raw data~\cite{wang2023bfu}.  It proposes an unlearning rate that removes the trade-off between erasing data and maintaining global model accuracy. The BFU-SS global model attains an accuracy of $97.68\%$ on the MNIST's test dataset while unlearning $10\%$ of data.


\subsection{Efficient Unlearning}
In addition to model accuracy, efficiency is one of the metrics for evaluating federated unlearning algorithms. To avoid communication costs and complex coordination in retraining, efficient federated unlearning methods should be capable of updating global models quickly and consuming less energy than retraining. For instance, the FedRecovery algorithm utilizes differential privacy by introducing tailored Gaussian noise to model updates to minimize the difference between the original and unlearned model after removing specific data~\cite{zhang2023fedrecovery}. It ensures that the unlearned model's accuracy remains statistically similar to a retrained model while avoiding excessive computational retraining costs. The time consumed by the FedRecovery algorithm is primarily attributed to calculating gradient residuals and managing the storage and retrieval of cached data. More precisely, this process takes approximately $1$ second compared to the $679.1$ seconds needed for retraining. Furthermore, FedEraser uses historical updates to restore previous model~\cite{liu2021federaser}. Using historical parameter updates for re-calibration accelerates the process of removing the global model, resulting in a $3.4$× improvement in time consumption for the Adult dataset, and decreasing the reconstruction time of the MNIST and Purchase datasets by $4.8$× and $4.1$×, respectively.



\subsection{Adaptation to Real-Time Data Dynamics}
Efficient federated unlearning algorithms also emphasize the capability of adaptation, since models are changing constantly in response to real-time data dynamics, such as evolving data distributions, as well as removing outdated and wrong data. This is demonstrated in the TF-IDF algorithm used for channel discrimination in CNNs~\cite{wang2022federated}. It effectively adjusts the model to the updated dataset without extensive retraining, focusing on channels relevant to the data categories to be unlearned. A subsequent fine-tuning step mitigates any accuracy loss, ensuring the model remains accurate and aligned with the new data distribution after unlearning. In terms of efficiency, TF-IDF significantly speeds up the unlearning process by $8.9$× for the ResNet model and $7.9$× for the Visual Geometry Group (VGG) model on the CIFAR-10 dataset, all without any loss of accuracy, in comparison to training the models from scratch. At the same time, FedLU deals with the discrepancy between local optimization and global convergence by supporting local models to independently forget and aggregate global information. This enables local models to adjust by forgetting outdated knowledge and controlling the trade-off between learning new data and unlearning obsolete knowledge ~\cite{zhu2023heterogeneous}.



\subsection{Mitigating Security Risks}
Federated unlearning techniques should ensure not only the efficient removal of data but also the protection from the possibility of privacy invasion during the process. Moreover, the federated unlearning creates changes in the training data such that there are different model versions before and after unlearning. This variation can expose the system to data poisoning threats, including such as Membership Inference Attacks (MIAs), Model Inversion Attacks, and Gradient Leakage Attacks~\cite{wang2023federated}. In dealing with MIAs, the defense strategy is to minimize the impact of individual data samples on the output of the model. This has been shown by the Exact-Fun algorithm which utilizes a gradient descent algorithm for model updates during unlearning~\cite{xiong2023exact}. It adds noise to the update process to hide the influences of the data being unlearned. This is an unwanted noise that messes up the traceability of the data inside the model, thus, making the data protected.


\subsection{Scalability in Large-Scale Systems}
Apart from the above capabilities, in large-scale federated learning systems, it is crucial for federated unlearning methods not to overload the network or the central server,  ensuring timely updates aligned with data privacy requirements. The FFMU algorithm is designed for resource-limited edge devices in federated settings~\cite{che2023fast}. Particularly, FFMU utilizes tools, such as the Nemytskii operator, to facilitate efficient unlearning in local models. This algorithm supports concurrent training and unlearning, crucial for managing a large-scale network of clients. By optimizing local models for unlearning, FFMU reduces the computational demands, enhancing scalability and enabling rapid response to unlearning requests without stressing any part of the system. Additionally, the KNOT framework~\cite{su2023asynchronous} utilizes a clustered aggregation mechanism to minimize retraining costs, targeting only specific clusters for unlearning while the rest of the system operates smoothly, optimizing resource usage. Thus, FFMU employs nonlinear functional analysis to map local models to global outcomes to avoid the time-consuming process of sequential unlearning and retraining, whereas KNOT strives to optimize the unlearning process by organizing data clusters to minimize computational and communication overhead.


In summary, tailored noise is a very efficient method for dealing with security threats of federated unlearning algorithms. Moreover, storing historical parameters can effectively speed up the federated unlearning without retraining from scratch. Besides, federated unlearning is also applied to delete obsolete data and thereby ensure the actuality of federated learning systems.






==> chapters/9-chap-paper_table.tex <==
\begin{table*}[!h]
\centering
\resizebox{\textwidth}{!}{%
\small
\begin{tabularx}{\textwidth}{lll>{\raggedright\arraybackslash}Xlll}
\toprule
\textbf{Taxonomy}& \textbf{References} & \textbf{Perspective}  & \textbf{Main Techniques} & \textbf{DHP} &  \textbf{MA} & \textbf{Metrics}\\
\hline
\multirow{6}{*}{Client}    & \cite{yuan2023federated} & P4, P5 & Model reconstruction & \ding{51} &  \ding{51}  & C1, C3, C7 \\
 & \cite{su2023asynchronous} & P4, P6 & Clustering & \ding{51} &  \ding{51} & C1, C7 \\
 & \cite{zhang2023fedrecovery}&  P1, P3, P4 & \ding{172}Differential Privacy \ding{173}Model Reconstruction & \ding{51}  & \ding{51} & C1, C4, C7 \\
 & \cite{guo2023fast} & P3, P4 & Model Reconstruction & \ding{51} & \ding{51} & C1, C7 \\
 & \cite{zhao2023federated} & P2, P3, P4 & \ding{172}Knowledge Erasure \ding{173}Memory Guidance & \ding{55} & \ding{51} & C1, C3, C7 \\  \hline

\multirow{6}{*}{Sample}
& \cite{xia2023fedme} & P3 & Memory Evaluation and Erasure &  \ding{55} & \ding{51} & C1, C4  \\ 
& \cite{zhu2023heterogeneous} & P6 & \ding{172}Knowledge Distillation \ding{173}Interference and Decay Theory & \ding{55} & \ding{55} & C1\\
& \cite{wang2023bfu} & P3 & \ding{172}Bayesian Inference \ding{173}Parameter Self-sharing & \ding{55} & \ding{51} & C1, C2, C3, C7  \\
& \cite{che2023fast} & P4 & \ding{172}Nemytskii Operator \ding{173}Manifolds & \ding{55} & \ding{51} & C1, C7\\
& \cite{wang2023edge} & P3, P6 & \ding{172}Edge Caching \ding{173}Model Decomposition  & \ding{55} & \ding{51} & C1, C7\\
& \cite{xiong2023exact} & P4, p6 & $\alpha$-quantization &\ding{55} & \ding{51}& C1, C4, C7\\
\hline

\multirow{2}{*}{Class}
& \cite{wang2022federated} & P3, P4 & Channel Pruning & \ding{55}  &  \ding{55} & C1, C4, C7\\
& \cite{zhao2023federated} & P2, P3, P4 & \ding{172}Knowledge Erasure \ding{173}Memory Guidance & \ding{55} & \ding{51} & C1, C3, C7 \\
\hline
\end{tabularx}}
% \vspace{-2mm}
\caption{Comparison of some prominent Federated Unlearning (FU) methods. Privacy (P1), Security (P2), Model Utility (P3), Computation Efficiency (P4), Storage Efficiency (P5), Communication Efficiency (P6), Incentive Mechanism Design (P7); Performance-based Metrics (C1), Model distribution-based Metrics (C2), Poisoning Attack (C3), Membership Inference Attack (C4), Watermark (C5), Erroneous Memory (C6), Efficiency (C7); Depend on Historical Parameters (DHP), Model Agnostic (MA).}
\label{literatures}
\end{table*}

